RoboPol: Do optical polarization rotations occur in all blazars?

We present a new set of optical polarization plane rotations in blazars, observed during the third year of operation of RoboPol. The entire set of rotation events discovered during three years of observations is analysed with the aim of determining whether these events are inherent in all blazars. It is found that the frequency of the polarization plane rotations varies widely among blazars. This variation cannot be explained either by a difference in the relativistic boosting or by selection effects caused by a difference in the average fractional polarization. We conclude that the rotations are characteristic of a subset of blazars and that they occur as a consequence of their intrinsic properties.

==> commands.tex <==
\newcommand{\nm}[1]{\textrm{#1}}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\abs}[1]{\vert #1 \vert}
\newcommand{\avg}[1]{\left\langle #1 \right\rangle}
\newcommand{\dg}{^{\circ}}
\newcommand{\fign}[1]{Figure~\ref{#1}\xspace}
\newcommand{\ditto}{$- \prime \prime -$}
